Multiscale Analysis of Count Data through Topic Alignment

Topic modeling is a popular method used to describe biological count data. With topic models, the user must specify the number of topics $K$. Since there is no definitive way to choose $K$ and since a true value might not exist, we develop techniques to study the relationships across models with different $K$. This can show how many topics are consistently present across different models, if a topic is only transiently present, or if a topic splits in two when $K$ increases. This strategy gives more insight into the process generating the data than choosing a single value of $K$ would. We design a visual representation of these cross-model relationships, which we call a topic alignment, and present three diagnostics based on it. We show the effectiveness of these tools for interpreting the topics on simulated and real data, and we release an accompanying R package, alto, available at https://lasy.github.io/alto.

==> purgatory.tex <==

%These results have the following interpretations.
%The score is maximized if a node's descendants descend solely from it, as we expect to see for nodes corresponding to true topics or mixtures of true topics.
%We have defined the refinement score so that it is equal to 1 if all the edge weights are equal and there is no relationship between the topics estimated at the different levels.
%The score is smallest for nodes that don't have any descendants that recognize them as parents at all.

  % the supplemental material includes ten replicates each of alignments performed either on data coming from an LDA model with $K = 5$ and the same values of $N$ and $D$ as above, or from a null model in which the topic proportion vector for each sample is drawn independently from a $\text{Dir}(\mathbf 1_D)$. We show both product and transport alignments and color by path, coherence, and refinement. The results are in line with the summaries given in Figure \ref{fig:gradient-combined}. We see clear differences in all of the diagnostics for the data generated under the null model vs. the data generated under the topic model with $K = 5$. The number of paths when $K = 5$ generally plateaus at 5, while in the null model the number of paths continues to increase as we add more topics. The coherence scores are all around 0 and the refinement scores are all around 1 in the null model. In the topic model with $K = 5$, for $K \leq 5$ we have moderately high coherence scores, but when $K > 5$ some of the topics have coherence scores very close to zero. These topics are presumably spurious and should not be taken to represent the true structure in the data. Similarly, for the refinement scores we see that for $K \leq 5$, the refinement scores are not that high, but for $K > 5$ we start to see some nodes with very high refinement scores and some nodes with very low refinement scores. The nodes with very low refinement scores are the same as those with very low coherence scores and represent spurious topics. The nodes with the higher refinement scores are more likely to represent true topics or true structure in the data. 
  
   % panel shows that the number of paths increases more gradually as a function of $K$, and that, across simulation replicates, there is more variation in the number of paths.
   
   
%We focus on the case that topics are derived from a sequence of models with increasing $K$. Then, we can identify each model $m$ with a unique scale $k$ and set $M = \{1, \dots, K\}$. This choice of sequential comparisons makes it possible to perform a multiscale analysis. Topics that, for models with large $k$, can distinguish between subtle variations in samples, can be related overview topics from models with small $k$.

"context"

- topics models: what they are and how they are used

"specific topic of \& motivation for paper"

- choosing the number of topics, interpreting a large number of topics
- gap: cross-validation may only provide an ideal K, but does not allow to navigate the trade-off between interpretability and expressivity

- introduce the potential "problems" (= each simulations) that you may not be able to uncover with cross-validation or hierarchical LDA.
- Make this a clear bullet list, introduce the subsection with examples


"our contribution (summary)"

- alignment of topics across K
- diagnostic metrics
- implementation of an R package

"content"

- Describing the methods and diagnotic metrics
- Show the results of simulated data for each of the situation described above
- Show the results on case study: the vaginal microbiome data
- Brief description of the package functions and workflow



[depending on where we submit (microbiology vs more general journal): 1-2 sentences on the relevance of microbiome for health and environmental studies - something along the line of] 

In the past decade [or two decades?], our (re)discovery of microbial communities via high-throughput sequencing and our improve understanding of its interaction with other species or tissues have highlighted its critical role for health of individuals and ecosystems [cite a book]. [+a few examples such as] For example, the gut microbiome was shown to play a critical role in xxx (find the landmark study in nutrition) and explain the inter-individual differences in glycemic responses to various sugars (Zeevi et al.,Cell), non-Lactobacillus dominated vaginal microbiomes were shown to be associated with the risk of preterm birth [cite] and [example in environmental biology]

[paragraph on how the microbiome composition is typically measured]
The microbiome composition is typically assessed by sequencing a specific region of the 16S rRNA gene of bacteria [cite]. This region shows specific variations that allow to identify bacterial species at various taxonomic levels depending on the bacteria. For example, specific mutations in this region may allow the identification of well studied bacteria at the genus, species or even strain level, providing a high resolution description of microbiomes.

\subsection{"specific topic of paper"}

[paragraph on how microbiome data is typically analyzed]
sequencing results: table of ASV counts for each sample. The number of ASV is typically very large, (order of 1000-10,000), often larger than the number of samples.

Consequently, it is often useful to use dimension reduction techniques, such as PCA/PCoA or clustering, to find features of the microbiome that may be associated with specific outcomes of interest.

Recently, topic analysis, or Latent Dirichlet Allocation (LDA), has been used to model microbiome composition. Topic analysis was introduced by Blei et al [cite] to identify topics in written documents. This statistical method is particularly suited to model microbiome composition because xxxx
Pros: dimension reduction, interpretable, mixed membership (so more flexible than clustering)

[explain a bit more about topic models, betas, gammas, maybe add an illustration?]

However, similarly to clustering methods, topic models are defined [better word than defined?] by a few key hyper-parameters such as the number of topic ($K$) or the expected sparsity of topics ($\alpha$). Scientists relying on topic models or on clustering are faced with the task of choosing an appropriate value for these hyper-parameters.

\subsection{"gap in knowledge, motivations"}

While several solution based on cross-validation (clustering and topic analyses) [cite] or based on the tightness of clusters (clustering) [cite] have been proposed to choose the appropriate number of topic or clusters, these methods often solely provide an optimal value without providing context or knowledge on the clusters or the topics. [that's not very well explained - let's think how we can explain better what they lack and what we offer]

For example, none of these solutions provide a method to evaluate if some clusters or some topics might be more robust than others nor how a change of parameter impacts the clustering or the topic composition.


\subsection{"overview of proposed methods, results and conclusions"}

Here, we propose a method to align topics across $K$ such that robust topics or clusters might be identified. 





We developed an interactive R package \verb alto implementing our method to align and identify robust topics, and applied our method on synthetic and real-world data (here, we used microbiome data) to evaluate its performance and discuss how results may be interpreted.

The problem of comparing and contrasting LDA models fitted across a range of K is related to the large literature on selecting “퐾” in various unsupervised contexts.  For example,() discuss436 selection of the number of clusters in clustering algorithms, and() give methods for selecting the dimensionality in dimensionality-reduction problems. However, we view the problem of selecting an optimal model as distinct from comparing across an ensemble. 
The former question focuses on whether there are differences between models, the latter focuses on where. In this spirit, the proposed alignment technique has more in common with methodology for comparing clusterings WagnerandWagner(2007), visualmodelcriticism Gabryetal.(2019); Pregibon(1981), 442 and posterior predictive analysis Gelman(2004); GelmanandShalizi(2013), for example

Though the LDA model is flexible, it can be challenging to interpret, especially in settings where $K$ is large. Existing work has addressed this difficulty by either modifying the model’s generative mechanism or proposing improved visualization of the model’s output.
For example, \citep{singer2014interpretability} modify the original LDA mechanism by compartmentalizing interpretation across subsets of columns. Specifically, the original $D$ columns can be divided into a collection of user-specified blocks of dimension $\tilde{D}_{1}, \dots, \tilde{D}_{B}$ such that $\sum_{b}\tilde{D}_{b} = D$. Each block is modeled with its own topics,
% \item 
\begin{align*}
p\left(x_i \vert \left(\gamma_ib\right), B_{b}\right) = \prod_{b} p\left(x_{iD_{b}} \vert \gamma_{ib}, B_b\right)
\end{align*}
where the density within each block $b$ is modeled using LDA. Since each block can be viewed separately from the others, this approach can be more directly interpretable in many problems.
An alternative, proposed by \citep{blei2003hierarchical} modifies the generative mechanism by basing it on an interpretable tree structure. This approach begins by imagining a depth $L$ tree with topics $\left(\beta_{k}^{l}\right)_{k = 1}^{K_{l}}$ at nodes on level $l$ in the tree. Each sample $i$ is associated with a path $\nu_i$ from the root of the tree to a leaf. Simulate $\gamma_i \sim \Dir\left(\lambda_{\gamma} 1_L\right)$ giving mixture weights over nodes on this path. The sample’s counts are then drawn according to,
\begin{align*}
x_{i} \vert \gamma_i, \left(\beta_{k}^{l}\right)_{k, l} \sim \Mult\left(n_i, \sum_{l =1}^{L} \gamma_{il} \beta_{\nu_i\left(l\right)}\right)
\end{align*}
The model is completed by specifying a prior on paths $\nu_i$ and $\beta_{k}^{l}$. Briefly, the $\nu_{i}$ are induced through a nested Chinese Restaurant Process while the $\beta_{k}^{l}$ are drawn from a Dirichlet, we refer the reader to \citep{blei2003hierarchical} for details. Note that, since the $\beta_k^{l}$ near the root of the tree will be shared by many samples, they tend to concentrate most of their probability on the most common terms. Topics near the leaves will account for systematic, but rarer, departures from these coarser, foundational topics. This multiresolution structure can facilitate interpretation, allowing construction of tree visualizations with each topic's most common words placed within nodes.

Possible titles (* = my favorite; @ = Laura's favorite),

\begin{enumerate}
\item Characterizing Fine-Grained Variation in Topic Models using Alignment (@)
\item Alto: An R Package for Aligning Topics at Varying Resolution (*, @)
\item Alignment Strategies for Resolving Differences in Topic Models
\item Interpreting Topic Models by Modulating Topic Resolution
\item Interpreting Topic Models by Aligning Topics at Varying Resolution (@)
\item Improving Topic Model Interpretability through Refinement
\item Choosing and Comparing K: Strategies for Topic Models (but we don’t really do this)
\item Hierarchical Interpretations from Flat Topic Models
\item Multiresolution Analysis of Count Data using Topic Alignment (*, @)
\item Comparing Ks in Topic Analysis using Alignment (*)
\end{enumerate}


\section{Results}


\subsection{Real-world dataset: vaginal microbiome samples}



[FIGURE: topic "Sankey" for different Ks]

[FIGURE: topic "Sankey" for different alphas (on a different dataset?)]

[FIGURE: topic "Sankey" for different modalities (on a different dataset?)]


\section{Discussion}


    

\section{Methods and Materials}

\subsection{Topic analyses}

% [Write down briefly the method and explain which package we used.]

Our methods for topic alignment are built on the solutions that result from fitting an LDA model.
We fit LDA using the {\tt topicmodels} package in R \cite{}.
% I don't know if you have different opinions on what to call things -- I'm using \Gamma, B, n, p, k, but they can be something different if that's more standard or if you prefer other notation.
The two matrices that are important to our later analyses are the sample composition matrices, which we will denote $\Gamma$, and the topic composition matrices, which we will denote $B$.
If we have $n$ documents, $p$ words, and $k$ topics, $\Gamma \in [0,1]^{n \times k}$, and $\Gamma_{ij}$ represents what fraction of document $i$ is composed of topic $j$.
We will similarly have $B \in [0,1]^{p \times k}$, the column sums of $B$ will be equal to 1, and the $j$th column of $B$ is a probability vector describing the word composition of the $k$th topic.

\subsection{Topic alignment based on sample composition (gammas)}

% Suggest having more biology intuition/examples about what the interpretations are
Our aim is to quantify the extent to which a topic in one LDA solution is aligned with a topic in another LDA solution, using the sample composition matrices corresponding to the two solutions.
% I don't know if you all like having motivations for the methods here, or if you like this particular motivation. It's kind of long, and I could see someone making the case that it's better to just say what we want to do and assert that it's reasonable.
To do this, we proceed by analogy to hard clustering.
Suppose that $\Gamma_1 \in \{0,1\}^{n \times k_1}$ and $\Gamma_2 \in \{0,1\}^{n \times k_2}$ are matrices such that $(\Gamma_1)_{ij}$ is the indicator that sample $i$ is a member of the $j$th cluster in clustering solution 1, and similarly for $\Gamma_2$ and clustering solution 2.
We can then take $(\Gamma_1^T \Gamma_1)^{-1} \Gamma_1^T \Gamma_2$ to be a matrix whose $ij$th element gives the similarity between cluster $i$ in clustering solution 1 and cluster $j$ in clustering solution 2.
The intuition here is that $(\Gamma_1^T \Gamma_2)_{ij}$ is the number of samples that are members of both cluster $i$ in clustering solution 1 and cluster $j$ in clustering solution 2.
$(\Gamma_1^T \Gamma_1)$ is a diagonal matrix whose $ii$th element is the number of samples present in cluster $i$ in clustering solution 1.
Therefore, $(\Gamma_1^T \Gamma_1)^{-1} \Gamma_1^T \Gamma_2$ is a matrix whose rows sum to 1, and the $i$th row can be interpreted as a vector of alignment scores between cluster $i$ in clustering solution 1 and all of the clusters in clustering solution 2.

To adapt this intuition to topic models, where every sample is assigned a weight for each document instead of being classified as being in exactly one topic, we can do something very similar.
Suppose now that $\Gamma_1 \in [0,1]^{n \times k_1}$ and $\Gamma_2 \in [0,1]^{n \times k_2}$ are the sample composition matrices for two LDA solutions.
For topic alignment scores, we can use
\begin{align*}
  \text{diag}(\Gamma_1^T \Gamma_2 \mathbf 1_{k_2})^{-1} \Gamma_1^T \Gamma_2.
\end{align*}
The $\text{diag}(\Gamma_1^T \Gamma_2 \mathbf 1_{k_2})^{-1}$ part of the expression is analogous to $(\Gamma_1^T \Gamma_1)^{-1}$ from hard clustering, and serves to ensure that the row sums of the resulting expression are all equal to 1.
The $\Gamma_1^T \Gamma_2$ part of the expression is exactly the same as its counterpart in hard clustering, and serves as an ``unnormalized'' measure of the similarity between two topics.
As before, the $i$th row of this matrix gives us a vector of alignment scores whose sum is 1 and that tells us about the similarity between topic $i$ in LDA solution 1 and all of the topics in LDA solution 2.


\subsection{Topic alignment based on topic composition (betas)}

Our second aim is to quantify the extent to which a topic in one LDA solution is aligned with a topic in another LDA solution, using the topic composition matrices corresponding to the two solutions.

Our strategy is... and is motivated by...

[write down how the weights and normalized weights are computed - optimization problem]

[LSY: should we have how the synthetic data are simulated in the method? And just keep the performance on simulated data in the results? I'd move items 1-5 that Kris wrote (I assume it was Kris) in the simulation part to the Methods]


Each rectangle corresponds to one topic, and their associated models increase in resolution proceeding from left to right. The height of a topic is proportional to the total document mass of that topic, i.e. $\sum_i \gamma_{ik}^{(m)}$. The width of links between pairs of topics encodes their alignment. \textit{Right}: The topic signatures $\beta_{k}^{(m)}$ associated with models $m$ with $K = 2$ to 10 topics. Topics with high alignments in the left plot have similar signatures on the right

The left side of each figure is a flow diagram, representing both the total mass across topics and the alignment weights $w\left(e\right)$. Each rectangle corresponds to a single topic, and its size corresponds to its mass $\sum_{i} \gamma_{ik}$. Vertical sections of the flow correspond to fitted models. The model with only one topic is given on the far left, while the model with 10 topics is on the far right. The width of links encodes the topic alignment weights $w\left(e\right)$. Topics and edges are colored to show paths.

The right side of each figure gives topic weights $\beta_{kd}$ across dimensions $d$. Each column corresponds to one topic, each row is a dimension, and the size of each circle is proportional to $\beta_{kd}$.  The colors of topics correspond to those in the flow. Sets of topics corresponding to one model are grouped into panels. Topic-dimension combinations with $\beta_{kd} < 0.001$ are ommitted, to prevent cluttering the display. Dimensions $d$ are sorted according to the measure
\begin{align*}
\text{Distinctiveness}\left(d\right) := \min_{l \neq k} \beta_{kd} \log \frac{\beta_{kd}}{\beta_{ld}}+\beta_{ld}-\beta_{kd},
\end{align*}
which is the same as that proposed by \citep{dey2017visualizing}, with the exception that now $k, l$ vary over topics from multiple models. Only the 25 most distinctive dimensions are displayed.

 When using transport alignment, there is a detectable increase in the number of estimated key topics for $K \geq 5$; however, the rate of increase is much slower than for $K < 5$.
Therefore, a practical rule-of-thumb would be to place higher trust in topics that have high refinement scores after the upper envelope plateaus. Therefore, a drop-off in refinement scores can be used to detect the introduction of spurious topics.
Further, for larger $K$, the overall fraction of points with low refinement scores increases.

This means that if we are considering an edge connecting nodes at $k < k'$, where $k \le k_0$, the nodes connected by the edge could either be true topic/true topic, mixture of topics/true topic, true topic/arbitrary split of that topic, or mixture of topics/arbitrary split of one of the topics in the mixture. In all of these cases, we expect the node at $k'$ to have only one parent at level $k$. On the other hand, if we are considering an edge connecting nodes at $k$ and $k'$, where $k_0 < k < k'$, then in addition to all of the possibilities listed before, we can have the nodes at the two levels be different arbitrary splits of the same topic. In that case, if we expect a different arbitrary split in the different levels, we expect the node at $k'$ to have more than one parent in level $k$.


